Multilinear PageRank

In this paper, we first extend the celebrated PageRank modification to a higher-order Markov chain. Although this system has attractive theoretical properties, it is computationally intractable for many interesting problems. We next study a computationally tractable approximation to the higher-order PageRank vector that involves a system of polynomial equations called multilinear PageRank, which is a type of tensor PageRank vector. It is motivated by a novel "spacey random surfer" model, where the surfer remembers bits and pieces of history and is influenced by this information. The underlying stochastic process is an instance of a vertex-reinforced random walk. We develop convergence theory for a simple fixed-point method, a shifted fixed-point method, and a Newton iteration in a particular parameter regime. In marked contrast to the case of the PageRank vector of a Markov chain where the solution is always unique and easy to compute, there are parameter regimes of multilinear PageRank where solutions are not unique and simple algorithms do not converge. We provide a repository of these non-convergent cases that we encountered through exhaustive enumeration and randomly sampling that we believe is useful for future study of the problem.

==> dgleich-extra.tex <==

\usepackage{ushort}
\newcommand{\cel}[1]{\ushort{#1}}
\newcommand{\cbmat}[1]{\left\{ \begin{matrix} #1 \end{matrix} \right\}}
\newcommand{\csbmat}[1]{\left\{\! \begin{smallmatrix} #1
\end{smallmatrix} \! \right\}}
%\newcommand{\csbmat}[1]{\underline{\sbmat{#1}}}
\newcommand{\smallmath}[1]{\begin{smallmatrix}#1\end{smallmatrix}}
\newcommand{\celm}[1]{\cel{\mat{#1}}}
\newcommand{\celv}[1]{\cel{\vec{#1}}}


\newcommand{\calpha}{\ensuremath{\cel{\alpha}}}
\newcommand{\cbeta}{\ensuremath{\cel{\beta}}}
\newcommand{\clambda}{\ensuremath{\cel{\lambda}}}

\newcommand{\cone}{\ensuremath{\cel{1}}}
\newcommand{\ca}{\ensuremath{\cel{a}}}
\newcommand{\cb}{\ensuremath{\cel{b}}}
\newcommand{\cc}{\ensuremath{\cel{c}}}
\newcommand{\cd}{\ensuremath{\cel{d}}}
\newcommand{\ce}{\ensuremath{\cel{e}}}
\newcommand{\cf}{\ensuremath{\cel{f}}}
\newcommand{\cg}{\ensuremath{\cel{g}}}
\newcommand{\ch}{\ensuremath{\cel{h}}}
\newcommand{\ci}{\ensuremath{\cel{i}}}
\newcommand{\cj}{\ensuremath{\cel{j}}}
\newcommand{\ck}{\ensuremath{\cel{k}}}
\newcommand{\cl}{\ensuremath{\cel{l}}}
\newcommand{\cm}{\ensuremath{\cel{m}}}
\newcommand{\cn}{\ensuremath{\cel{n}}}
\newcommand{\co}{\ensuremath{\cel{o}}}
\newcommand{\cp}{\ensuremath{\cel{p}}}
\newcommand{\cq}{\ensuremath{\cel{q}}}
%\newcommand{\cr}{\ensuremath{\cel{r}}}
\newcommand{\cs}{\ensuremath{\cel{s}}}
\newcommand{\ct}{\ensuremath{\cel{t}}}
\newcommand{\cu}{\ensuremath{\cel{u}}}
\newcommand{\cv}{\ensuremath{\cel{v}}}
\newcommand{\cw}{\ensuremath{\cel{w}}}
\newcommand{\cx}{\ensuremath{\cel{x}}}
\newcommand{\cy}{\ensuremath{\cel{y}}}
\newcommand{\cz}{\ensuremath{\cel{z}}}


\newcommand{\cA}{\ensuremath{\cel{A}}}
\newcommand{\cB}{\ensuremath{\cel{B}}}
\newcommand{\cC}{\ensuremath{\cel{C}}}
\newcommand{\cD}{\ensuremath{\cel{D}}}
\newcommand{\cE}{\ensuremath{\cel{E}}}
\newcommand{\cF}{\ensuremath{\cel{F}}}
\newcommand{\cG}{\ensuremath{\cel{G}}}
\newcommand{\cH}{\ensuremath{\cel{H}}}
\newcommand{\cI}{\ensuremath{\cel{I}}}
\newcommand{\cJ}{\ensuremath{\cel{J}}}
\newcommand{\cK}{\ensuremath{\cel{K}}}
\newcommand{\cL}{\ensuremath{\cel{L}}}
\newcommand{\cM}{\ensuremath{\cel{M}}}
\newcommand{\cN}{\ensuremath{\cel{N}}}
\newcommand{\cO}{\ensuremath{\cel{O}}}
\newcommand{\cP}{\ensuremath{\cel{P}}}
\newcommand{\cQ}{\ensuremath{\cel{Q}}}
\newcommand{\cR}{\ensuremath{\cel{R}}}
\newcommand{\cS}{\ensuremath{\cel{S}}}
\newcommand{\cT}{\ensuremath{\cel{T}}}
\newcommand{\cU}{\ensuremath{\cel{U}}}
\newcommand{\cV}{\ensuremath{\cel{V}}}
\newcommand{\cW}{\ensuremath{\cel{W}}}
\newcommand{\cX}{\ensuremath{\cel{X}}}
\newcommand{\cY}{\ensuremath{\cel{Y}}}
\newcommand{\cZ}{\ensuremath{\cel{Z}}}


\newcommand{\cva}{\ensuremath{\celv{a}}}
\newcommand{\cvb}{\ensuremath{\celv{b}}}
\newcommand{\cvc}{\ensuremath{\celv{c}}}
\newcommand{\cvd}{\ensuremath{\celv{d}}}
\newcommand{\cve}{\ensuremath{\celv{e}}}
\newcommand{\cvf}{\ensuremath{\celv{f}}}
\newcommand{\cvg}{\ensuremath{\celv{g}}}
\newcommand{\cvh}{\ensuremath{\celv{h}}}
\newcommand{\cvi}{\ensuremath{\celv{i}}}
\newcommand{\cvj}{\ensuremath{\celv{j}}}
\newcommand{\cvk}{\ensuremath{\celv{k}}}
\newcommand{\cvl}{\ensuremath{\celv{l}}}
\newcommand{\cvm}{\ensuremath{\celv{m}}}
\newcommand{\cvn}{\ensuremath{\celv{n}}}
\newcommand{\cvo}{\ensuremath{\celv{o}}}
\newcommand{\cvp}{\ensuremath{\celv{p}}}
\newcommand{\cvq}{\ensuremath{\celv{q}}}
\newcommand{\cvr}{\ensuremath{\celv{r}}}
\newcommand{\cvs}{\ensuremath{\celv{s}}}
\newcommand{\cvt}{\ensuremath{\celv{t}}}
\newcommand{\cvu}{\ensuremath{\celv{u}}}
\newcommand{\cvv}{\ensuremath{\celv{v}}}
\newcommand{\cvw}{\ensuremath{\celv{w}}}
\newcommand{\cvx}{\ensuremath{\celv{x}}}
\newcommand{\cvy}{\ensuremath{\celv{y}}}
\newcommand{\cvz}{\ensuremath{\celv{z}}}

\providecommand{\cmA}{\ensuremath{\celm{A}}}
\providecommand{\cmB}{\ensuremath{\celm{B}}}
\providecommand{\cmC}{\ensuremath{\celm{C}}}
\providecommand{\cmD}{\ensuremath{\celm{D}}}
\providecommand{\cmE}{\ensuremath{\celm{E}}}
\providecommand{\cmF}{\ensuremath{\celm{F}}}
\providecommand{\cmG}{\ensuremath{\celm{G}}}
\providecommand{\cmH}{\ensuremath{\celm{H}}}
\providecommand{\cmI}{\ensuremath{\celm{I}}}
\providecommand{\cmJ}{\ensuremath{\celm{J}}}
\providecommand{\cmK}{\ensuremath{\celm{K}}}
\providecommand{\cmL}{\ensuremath{\celm{L}}}
\providecommand{\cmM}{\ensuremath{\celm{M}}}
\providecommand{\cmN}{\ensuremath{\celm{N}}}
\providecommand{\cmO}{\ensuremath{\celm{O}}}
\providecommand{\cmP}{\ensuremath{\celm{P}}}
\providecommand{\cmQ}{\ensuremath{\celm{Q}}}
\providecommand{\cmR}{\ensuremath{\celm{R}}}
\providecommand{\cmS}{\ensuremath{\celm{S}}}
\providecommand{\cmT}{\ensuremath{\celm{T}}}
\providecommand{\cmU}{\ensuremath{\celm{U}}}
\providecommand{\cmV}{\ensuremath{\celm{V}}}
\providecommand{\cmW}{\ensuremath{\celm{W}}}
\providecommand{\cmX}{\ensuremath{\celm{X}}}
\providecommand{\cmY}{\ensuremath{\celm{Y}}}
\providecommand{\cmZ}{\ensuremath{\celm{Z}}}


==> preamble.tex <==
% definitions used by included articles, reproduced here for 
% educational benefit, and to minimize alterations needed to be made
% in developing this sample file.

\usepackage{dgleich-setup}
\usepackage{dgleich-math}
\renewcommand{\mat}{\boldsymbol}
%\usepackage{textcase}
%\usepackage{graphicx}
%\usepackage{xcolor}
\usepackage{epstopdf}
%\usepackage{url}
%\usepackage{tabularx}
%\usepackage{paralist}
\usepackage{subfigure}

\let\oldthebibliography=\thebibliography
\let\oldendthebibliography=\endthebibliography

\usepackage[square]{natbib}
\renewcommand{\cite}{\citep}

\let\thebibliography=\oldthebibliography
\let\endthebibliography=\oldendthebibliography

  \providecolor{theblue}{RGB}{0,0,180}%
  \RequirePackage[colorlinks,pdfdisplaydoctitle
      ,citecolor=theblue
      ,linkcolor=theblue
      ,urlcolor=theblue
      ,hyperfootnotes=false,pagebackref]{hyperref}%
%% Configure backreference from bibliography to pages in hyperref
\renewcommand*{\backref}[1]{}%
\renewcommand*{\backrefalt}[4]{%
  \ifcase #1 %
    No citations.%
  \or
    Cited on page #2.%
  \else
    Cited on pages #2.%
  \fi
}%



\input{dgleich-extra}


% some definitions of bold math italics to make typing easier.
% They are used in the corollary.

%\def\bfE{\mbox{\boldmath$E$}}
%\def\bfG{\mbox{\boldmath$G$}}
